Few-Shot Font Generation by Learning Fine-Grained Local Styles

Few-shot font generation (FFG), which aims to generate a new font with a few examples, is gaining increasing attention due to the significant reduction in labor cost. A typical FFG pipeline considers characters in a standard font library as content glyphs and transfers them to a new target font by extracting style information from the reference glyphs. Most existing solutions explicitly disentangle content and style of reference glyphs globally or component-wisely. However, the style of glyphs mainly lies in the local details, i.e. the styles of radicals, components, and strokes together depict the style of a glyph. Therefore, even a single character can contain different styles distributed over spatial locations. In this paper, we propose a new font generation approach by learning 1) the fine-grained local styles from references, and 2) the spatial correspondence between the content and reference glyphs. Therefore, each spatial location in the content glyph can be assigned with the right fine-grained style. To this end, we adopt cross-attention over the representation of the content glyphs as the queries and the representations of the reference glyphs as the keys and values. Instead of explicitly disentangling global or component-wise modeling, the cross-attention mechanism can attend to the right local styles in the reference glyphs and aggregate the reference styles into a fine-grained style representation for the given content glyphs. The experiments show that the proposed method outperforms the state-of-the-art methods in FFG. In particular, the user studies also demonstrate the style consistency of our approach significantly outperforms previous methods.

==> approach.tex <==
\section{Method}
In this section, we present the details of our FS-Font method. We first briefly review the few-shot font generation problem setup and introduce the overall framework of our method (\ref{Sec:3.0}). Next, we present the details of three crucial components of our approach, including the \textit{Style Aggregation Module} (SAM) (Sec. \ref{sec:3.1}), the Self-Reconstruction branch (Sec. \ref{sec:3.2}), and Reference Selection (Sec. \ref{sec:3.3}). 

\subsection{Problem Setting and Method Overview}\label{Sec:3.0}
In few-shot font generation, given a content glyph image $x_c$ with the content $c$ from a standard font and a $k$-shot reference glyph images with the style $s$: $R_{s}=\left\{y_i\right\}_{i=1}^k$, our goal is to generate a stylized image $I_o$ that have the content $c$ and style $s$ via a neural network generator $G$:
\begin{equation}
\label{eq:1}
I_o=G(x_c, \left\{y_i\right\}_{i=1}^k).
\end{equation} 
In training stage, we choose a standard font with $N$ glyphs $X = \{x_i\}^N_{i=1}$ and $L$ fonts with different styles $R = \{R_{s_t}\}^L_{s=1}$, where $R_{s_t} = \{y_i\}^N_{i=1}$. Each $(x_i,y_i)$ is a data pair with same content but different styles. 
%In our experiment with Chinese fonts, $L = 407$ and $N = 3396$.

The structure of the Generator is shown in Figure \ref{flowchart}. Given the sampled $R_s$ from $R_{s_t}$, the reference encoder $E_r$ first encodes $R_s$ into $k$-shot reference maps $F_r = \left\{f_{i}\right\}_{i=1}^k$, where $f_i$ is encoded from $y_i$. The content encoder $E_c$ extracts the content feature map $f_c$ from the input content image $x_c$. Our proposed SAM takes $F_r$ and $f_c$ as inputs, attends to the corresponding spatially local styles in the reference maps $F_r$ and aggregates the local styles into the target style map $f_{c, r} = SAM(f_c, F_r)$. In the end, the decoder $D$ decodes $f_{c, r}$ into the generated output image $I_o$. A multi-task projection discriminator\cite{miyato2018cgans} is employed to discriminate each generated image and real image. The discriminator outputs a binary classification of fake or real for each character's style and content category.


% In the training stage, the network $G$ is usually learned from a standard font with $n$ glyphs $\mathcal{D}_c = \left\{x_i\right\}^n_{i=1}$ and multiple fonts with $L$ different styles $\boldsymbol R_s = \{R_s\}^L_{s=1}$, where $R_s = \{{y}_i\}^{n}_{i=1}$. Each $(x_i,y_i)$ is a data pair with shared content but different styles. In our Chinese experiment, $L = 407$ and $n = 3363$.

% its corresponding font in $L$ different styles $\boldsymbol R_s = \{  \mathcal{R}_s^l\}^L_{l=1}$, where $\mathcal{R}_s^l = \{{y}^l_i\}^{n}_{i=1}$. Each $(x_i,y^l_i)$ is a data pair with shared content but different styles. It is worth noting that the $k$-shot reference glyphs $R$ has a different style than the styles in the training set $\boldsymbol R_s$.



\subsection{Style Aggregation Module}
\label{sec:3.1}

%The motivation of the Style Aggregation Module(SAM) is to recover the component details of the references. Commercial fonts require a target glyph has its components visually similar to those in references, if the corresponding components exists in references. A font designer would typically \textit{search} for the desired components in the references, \textit{copy} them, and \textit{paste} them to the corresponding location in target glyph. When the target component does not exists, the designer need to generalize the component by the style of references. To this end, inspired recent works on Transformers\cite{vaswani2017attention}, we design SAM to adaptively capture corresponding local styles from references to target. %As the local styles are directly extracted from references, no explicit disentanglement of content and style is needed.

An overview of the SAM is depicted in Figure \ref{fig:attention}. The core in SAM is a multi-head cross attention block that attends to spatially local styles from the reference maps $F_r$ and aggregates the reference styles into the fine-grained style representation for the given content image. For the $m$-th attention head, SAM learns a Query map $Q^m$ from content feature map $f_c$ and Key map $K^m$ from reference maps $F_r$, which achieves the spatial correspondence matrix $A^m$ between the pixels of $Q^m$ and $K^m$. A value map $V^m$ is simultaneously learned from $F_r$. Multiplying the correspondence matrix $A^m$ with the value map $V^m$ aggregates the local style styles into the target style $S^m$. As different head captures different information, we combine all the target styles together for decoding.

\begin{figure}   %注意，这里设置是关键
\centering
\includegraphics[width=\linewidth,scale=1.00]{latex/paper_images/SAM_chart2.png}
\caption{\textbf{The illustration of the Style Aggregation Module (SAM)}. We use multihead attention mechanism to calculate the spatial correspondence of content and references and generate the fine-grained feature map.}
\label{fig:attention}
\end{figure}


Formally, we reshape $f_c \in \mathbb{R}^ {c \times h \times w}$ into a sequence $\tilde{f_c} \in \mathbb{R}^ {c \times (h \cdot w)}$, where $(h, w)$ is the resolution of the feature map, $c$ is the number of channels. For the $m$-th head, after applying a linear layer $L^m_{query} \in \mathbb{R}^{c \times c^m}$, we acquire the query matrix $Q^m \in \mathbb{R}^{c^m\times (h \cdot w)}$. Meanwhile, the reference maps $F_r = \left\{f_{i}\right\}_{i=1}^k$ are reshaped and concatenated along the spatial dimension $(h, w)$, forming a reference sequence $\tilde{f}_r \in \mathbb{R}^ {c \times (k \cdot h \cdot w)}$. We multiply $\tilde{f}_r$ by two linear projections $L^m_{key}, L^m_{value} \in \mathbb{R}^{c \times c^m}$ and generate a key map $K^m$ and a value map $V^m$ that both are $\in \mathbb{R}^{c\times (k\cdot h \cdot w)}$:
\begin{equation}
\begin{split}
  &Q^m = L^m_{query}(\tilde{f_c}), \quad Q^m \in \mathbb{R}^{c^m \times (h \cdot w)}, \\
  &K^m = L^m_{key}(\tilde{f_r}),   \quad K^m \in \mathbb{R}^{c^m \times (k \cdot h \cdot w)}, \\
  &V^m = L^m_{value}(\tilde{f_r}), \quad V^m \in \mathbb{R}^{c^m \times (k \cdot h \cdot w)}. \\
  \end{split}
  \label{eq:key matrix}
\end{equation} 

We then compute a spatial correspondence matrix $A^m$ of which each element $A^m(u, v)$ is a pairwise feature correlation between content feature in position $u$ and reference feature in position $v$, calculated as follows: 

\begin{equation}
  A^m = \frac{Q^{m \top} K^m}{\sqrt{c^m}} \in \mathbb{R}^{hw \times khw},
  \label{eq:key matrix}
\end{equation}
where $c^m$ is the hidden dimension of $Q^m$ and $K^m$. The $1/\sqrt{c^m}$ factor follows Transformers\cite{vaswani2017attention} to prevent the magnitude of the dot product from growing extreme.

With the correspondence matrix $A^m$, we obtain the aggregated style from references by 
\begin{equation}
  S^m = softmax(A^m) V^{m\top} \in \mathbb{R}^{hw \times c^m}.
  \label{eq:key matrix}
\end{equation}

% we acquire the $m$-th target style from $m$-th attention head.
After permuting and reshaping $S^m$ into $\mathbb{R} ^ {c^m \times h \times w}$, we concatenate $M$ target styles and employ a linear projection $L_s \in \mathbb{R}^{(c^m \cdot M) \times c}$ to obtain target style $S$. The target style map $f_{c,r}$ is computed after concatenation between $S$ and content feature $f_c$, . The decoder $D$ decode it into the target image $I_o$ as follows:

\begin{equation}
\begin{split}
  &S = L_s(S^1 \circ S^2, ..., \circ S^M) \in \mathbb{R}^{c \times h \times w},\\  
  &I_{o} = D(f_{c,r}) = D(f_c \circ S),
  \label{eq:decode}
\end{split}
\end{equation}
where $\circ$ denotes concatenation operator and $M$ is the number of total attention heads.

\subsection{Self Reconstruction}
\label{sec:3.2}
% To achieve a highly style-consistent generated image can not solely rely on the proper aggregation of styles. It also relies on the expressivity of the styles to depict fine and local details of the references. 
To achieve a highly style-consistent glyph using SAM, it depends not only on the proper aggregation of styles, but also on the expressivity of the styles that depict fine and local details of the references. However,
the $k$-shot font generation setup is a hard-to-learn problem, as it requires the attention learns spatial correspondence from weakly correlated content-references pairs, which is sometimes confusing even for a human expert. 
Thus, besides the main branch of $k$-shot learning, we introduce an easy-to-learn Self-Reconstruction (SR) branch to boost the learning process. 

While the generator is trained in the above mentioned $k$-shot setup, for a given content input $x_c$, we have the ground truth image $I_{GT}$ to supervise the model training. Self Reconstruction is a parallel branch that shares the same model as the main branch during training. It takes $I_{GT}$ as the reference image $R_s=\left\{I_{GT}\right\}$, and its output $\tilde{I_o}$ is also supervised by $I_{GT}$ itself. In contrast to Eq. \ref{eq:1}, the generation process of this branch is 
\begin{equation}
\tilde{I_o}=G(x_c, I_{GT}).
\end{equation}

The detailed training setup can be found in Sec.\ref{sec:3.4}. In the SR branch, the content and reference images are strongly correlated. The spatial correspondence matrix can be easily learned as the strokes and the components' relationship between content and reference is clear. With the well-learned correspondence, the generator can be optimized with well-aligned gradients. As a result, the expressivity of depicting details can be further learned within our framework.

\subsection{Reference Selection}
\label{sec:3.3}

In previous works considering the decomposition of components like LF-Font\cite{park2020few}, reference characters that contain the same components as content character are randomly selected from the training set during each iteration. The model can hardly learn how to extract the right component-wise features with varying combinations of the reference set. Thus, we introduce a strategy to select a fixed reference set whose components cover most of the commonly used characters and design a content-reference mapping that fixes the combination of reference set for each character. To establish this mapping function, we firstly introduce a tree-structure component analyzer (TCA), as shown in Figure \ref{tree_analyzer}. Based on the analyzer, we can conveniently find the glyphs' conspicuous components, guaranteeing the efficiency of our subsequent steps.

\begin{figure}   %注意，这里设置是关键
\centering
\includegraphics[width=\linewidth,scale=1.0]{latex/paper_images/tree_v3.png}
\caption{\textbf{Tree-structure component analyzer (TCA).} We define components at the level 0, 1, and 2 as the conspicuous components, which are considered much easier be learned by our proposed model. To make the mapping process more sensible, the component's structure information is also taken into consideration.}
\label{tree_analyzer}
\end{figure}

\textbf{Reference set selection}. Initially, we select a small subset (typically including 100 characters) from a commonly-used character list, which offers the style references. This reference set should cover as many conspicuous-level components as possible. First, we analyze the characters by using the proposed tree-structure component analyzer. Once the character contains two or more new components, we add this character to our reference set. When the elements in the reference set reach their limits, we stop searching and obtain the style reference set and its corresponding contained components.% The selecting process can found in supplementary Algo. 1. 

% \begin{algorithm}
% \SetKwInOut{Input}{input}
% \SetKwInOut{Output}{output}
% \SetKwRepeat{Do}{do}{while}
% \Input{$X=\{x_i\}$: Common-used glyph list. \newline 
% $T=\{x_i:\chi_i\}$: Single-level decomposition look-up table. $\chi_i \subset X$. \newline
% $C$: Conspicuous-level component set. \newline
% ${N}_{ref}$: Max capacity of Reference set. \newline
% $d$: Max search depth in TCA.
% }
% \Output{$\hat{U}$: Reference set. \newline
% $\hat{C}$: All components which $U$ can cover.
% }
% \SetKwFunction{FMain}{searchComponents}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$x_i$}}{
%     $queue \leftarrow \{x_i\}$; $i \leftarrow 0$; $\hat{C} \leftarrow \emptyset $ \newline
%     \Repeat{$i \geq d$}{
%       $queue^{*} \leftarrow \emptyset $ \newline
%       \For{$x\in queue$}{
%         $queue^{*} \leftarrow queue^{*} \cup T(x) $ \newline
%         $\hat{C} \leftarrow T(x) \cap C $
%       }
%       $queue \leftarrow queue^{*}$; $i \leftarrow i+1$
%     }
%     \textbf{return} $\hat{C}$ \newline
% }
% \textbf{End Function}
% \newline

% \SetKwFunction{FMain}{Main}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{}}{
%     $\hat{U} \leftarrow \emptyset $; $\hat{C} \leftarrow \emptyset $ \newline
%     \For{$x_i\in X$}{
%         $c_i \leftarrow $ searchComponents($x_i$) \newline
%         \lIf{$\exists \hat{c} \in {c}_{i}$ s.t. $\hat{c} \notin \hat{C}$}{
%             $\hat{C} \leftarrow \hat{C} \cup {c}_{i}$, add $x_i$ to $\hat{U}$
%         }
%         \lIf{Len($\hat{U}$) $\geq$ ${N}_{ref}$}{\textbf{break}}
%     }
%     \textbf{return} $\hat{U}$, $\hat{C} $ \newline
% }
% \textbf{End Function}
% \caption{Reference set selection}
% \label{alg:refss}
% \end{algorithm}

\textbf{Content-reference mapping}. After completing the reference set selection, we then establish the mapping relations between content glyphs and style references. We propose a greedy process to find $k$-shot references for a glyph. In this process, we search the reference set for $k$ times to establish a mapping relation. During every searching step, we find the reference glyph that shares the most components with the target glyph. If there are multiple solutions, we select the optimal solution that has the most components with the same structure composition. After selection, we remove the reference from the reference set and continue the next searching step. By this process, we can determine every glyph's corresponding $k$-shot references.

%  \begin{table*}
%   \setlength\tabcolsep{12pt}
%   \centering
%   \begin{tabular}{lc|cccccc}
%       \toprule % 顶部的那个横线
%       \multicolumn{8}{c}{\textbf{Unseen Fonts Seen Characters}} \\ \cmidrule(lr){1-8}
%     %   \midrule % 中间那条线
%       Methods & Training & L1 loss $\downarrow$ & RMSE $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & User(Cls) \% $\uparrow$ & User(S) \% $\uparrow$ \\
%       \midrule
%       FUNIT & unpaired & 0.148 & 0.344 & 0.565 & 0.2543 & 86.0 & 0\\
%       DG-FONT & unpaired & 0.131 & 0.329 & 0.604 & 0.2154 & 92.4 & 0\\
%       MX-FONT & paired & 0.152 & 0.347 & 0.584 & 0.2291 & \textbf{97.4} & 0 \\
%       AGIS-NET & paired & 0.105 & 0.289 & 0.651 & 0.1865 & 97.2 & 0\\
%       LF-FONT & paired & 0.129 & 0.322 & 0.607 & 0.2006 & 93.4 & 0\\
%       Ours & paired & \textbf{0.097} & \textbf{0.268} & \textbf{0.671}& \textbf{0.1618} & 96.6 & 0\\
      
%       \midrule
%       \multicolumn{8}{c}{\textbf{Unseen Fonts Unseen Characters}} \\ \cmidrule(lr){1-8}
%       Methods & Training & L1 loss $\downarrow$ & RMSE $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & User(Cls) \% $\uparrow$ & User(S) \% $\uparrow$ \\ 
%       \midrule
%       FUNIT & unpaired & 0.152 & 0.345 & 0.532 & 0.2424 & 84.6 & 0\\
%       DG-FONT & unpaired & 0.141 & 0.341 & 0.573 & 0.2151 & 86.4 & 0\\
%       MX-FONT & paired & 0.153 & 0.352 & 0.573 & 0.2317 & 93.2 & 0\\
%       AGIS-NET & paired & 0.114 & 0.302 & 0.623 & 0.1877 & 89.8 & 0\\
%       LF-FONT & paired & 0.138 & 0.334 & 0.577 & 0.2018 & 90.6 & 0\\
%       Ours & paired & \textbf{0.106} & \textbf{0.283} & \textbf{0.642} & \textbf{0.1627} & \textbf{93.8} & 0\\
      
%       \bottomrule % 最下面那条线
%   \end{tabular}
%   \caption{\textbf{Qualitative comparison on UFUC and UFSC datasets}}
%   \label{comparison table}
% \end{table*}

% \begin{table*}
%   \setlength\tabcolsep{15pt}
%   \centering
%   \begin{tabular}{l|cccccc}
%       \toprule % 顶部的那个横线
%       \multicolumn{7}{c}{\textbf{Unseen Fonts Seen Characters}} \\ \cmidrule(lr){1-7}
%     %   \midrule % 中间那条线
%       Methods  & L1 loss $\downarrow$ & RMSE $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & User(C) \% $\uparrow$ & User(S) \% $\uparrow$ \\
%       \midrule
%       FUNIT \cite{liu2019few}  & 0.148 & 0.344 & 0.565 & 0.2543 & 86.0 & 0.3\\
%       DG-FONT \cite{xie2021dg}  & 0.131 & 0.329 & 0.604 & 0.2154 & 92.4 & 6.1\\
%       MX-FONT \cite{park2021multiple}  & 0.152 & 0.347 & 0.584 & 0.2291 & \textbf{97.4} & 8.4 \\
%       AGIS-NET \cite{gao2019artistic}  & 0.105 & 0.289 & 0.651 & 0.1865 & 97.2 & 5.2\\
%       LF-FONT \cite{park2020few}  & 0.129 & 0.322 & 0.607 & 0.2006 & 93.4 & 11.3\\
%       Ours  & \textbf{0.097} & \textbf{0.268} & \textbf{0.671}& \textbf{0.1618} & 96.6 & \textbf{68.7}\\
      
%       \midrule
%       \multicolumn{7}{c}{\textbf{Unseen Fonts Unseen Characters}} \\ \cmidrule(lr){1-7}
%       Methods  & L1 loss $\downarrow$ & RMSE $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & User(C) \% $\uparrow$ & User(S) \% $\uparrow$ \\ 
%       \midrule
%       FUNIT \cite{liu2019few}  & 0.152 & 0.345 & 0.532 & 0.2424 & 84.6 & 1.2 \\
%       DG-FONT \cite{xie2021dg}  & 0.141 & 0.341 & 0.573 & 0.2151 & 86.4 & 3.1\\
%       MX-FONT \cite{park2021multiple}  & 0.153 & 0.352 & 0.573 & 0.2317 & 93.2 & 11.2\\
%       AGIS-NET \cite{gao2019artistic}  & 0.114 & 0.302 & 0.623 & 0.1877 & 89.8 & 4.1\\
%       LF-FONT \cite{park2020few}  & 0.138 & 0.334 & 0.577 & 0.2018 & 90.6 & 13.3\\
%       Ours  & \textbf{0.106} & \textbf{0.283} & \textbf{0.642} & \textbf{0.1627} & \textbf{93.8} & \textbf{67.1}\\
      
%       \bottomrule % 最下面那条线
%   \end{tabular}
%   \caption{\textbf{Qualitative comparison on UFUC and UFSC datasets}}
%   \label{comparison table}
% \end{table*}


%With a generated reconstruction image $I_r$, an L1 loss and an adversarial loss will be computed as follows:

% \begin{equation}
% \begin{split}
%     &\mathcal{L}_{l1}^{recons} = \mathbb{E}_{\tilde{I_r} \in P_{g}, I \in P_{d}}\left[\lVert \tilde{I_r} - I\rVert_{1}\right] \\
%     &\mathcal{L}_{adv}^{recons} = \mathop{min}\limits_{G}\mathop{max}\limits_{D_{s,c}}\mathbb{E}_{I_o_r \in P_{g}, I \in P_{d}}[log(D_{s,c}(I)) \\
%       &+ log(1 - (D_{s,c}(I_o_r)))]
% \label{eq reconstruction loss}
% \end{split}
% \end{equation}

\subsection{Training}
\label{sec:3.4}
We train our model to generate the image $I_o$ from a content glyph image $x_c$ and a fixed set of reference glyph images $R_s$. In each iteration, the main branch and the SR branch generate $I_o$ and $\tilde{I_o}$ simultaneously and are supervised by the same losses. \textbf{FSFont} learns the reference encoder $E_r$, content encoder $E_c$, Style Aggregation Module and decoder $D$ with following losses: 1) Adversarial loss with multi-task discriminator. 2) L1 loss among $I_o$, $\tilde{I}_o$ and a paired ground truth image ${I_{GT}}$. 

\textbf{Adversarial loss}. Since we our aim is to generate visually high-quality images, we employ a multi-head projection discriminator \cite{miyato2018cgans} in framework. The loss function is represented as follows:

\begin{equation}
\begin{split}
  \mathcal{L}_{adv} & = \mathop{min}\limits_{G}\mathop{max}\limits_{D_{s,c}}\mathbb{E}_{I_{out} \in P_{g}, I_{GT} \in P_{d}}[log(D_{s,c}(I_{GT})) \\
  &+ log(1 - (D_{s,c}(I_{out})))] ,
  \label{eq GAN loss}
\end{split}
\end{equation}
where $D_{s,c}(\cdot)$ refers to the logit of the character $c$ and style $s$ from discriminator, $P_g$ denotes the set of generated images from both main branch and Self-Reconstruction branch. $I_{out}$ denotes $ \{I_o, \tilde{I}_o\}$ and $P_d$ denotes the set of real glyph images. \\

\textbf{L1 loss}. For learning the pixel-level consistency, we employ an L1 loss between generated images $I_{out}$ and ground truth images $I_{GT}$. 
\begin{equation}
  \mathcal{L}_{l1} = \mathbb{E}\left[\lVert I_{out} - I_{GT}\rVert_{1}\right].
  \label{eq GAN loss}
\end{equation}

\textbf{Overall objective loss}.
Combining all losses mentioned above, we train our whole framework by minimizing the following objective loss functions:
\begin{equation}
\begin{split}
  \mathcal{L}_{obj} = \lambda_{adv}\mathcal{L}_{adv} +  \lambda_{l1}\mathcal{L}_{l1}, %&+ \\ %\lambda_{recons}(\lambda_{l1}\mathcal{L}_{l1}^{recons} & + \mathcal{L}_{adv}^{recons}),
\label{eq:key matrix}
\end{split}
\end{equation}
%where $\lambda_{adv}$, $\lambda_{l1}$ and $\lambda_{recons}$ are hyperparameters to control the weight of each objective loss. We empirically set  $\lambda_{adv}=1$, $\lambda_{l1}=0.1$ and $\lambda_{recons}=1$ in our experiments.
where $\lambda_{adv}$ and $\lambda_{l1}$ are hyperparameters to control the weight of each objective loss. We empirically set  $\lambda_{adv}=1$ and $\lambda_{l1}=0.1$ in our experiments.
